SoK: Cross-Chain Bridging Architectural Design Flaws and Mitigations

Cross-chain bridges are solutions that enable interoperability between heterogeneous blockchains. In contrast to the underlying blockchains, the bridges often provide inferior security guarantees and have been targets of hacks causing damage in the range of 1.5 to 2 billion USD in 2022. The current state of bridge architectures is that they are ambiguous, and there is next to no notion of how different architectures and their components are related to different vulnerabilities. Throughout this study, we have analysed 60 different bridges and 34 bridge exploits in the last three years (2021-2023). Our analyses identified 13 architectural components of the bridges. We linked the components to eight types of vulnerabilities, also called design flaws. We identified prevention measures and proposed 11 impact reduction measures based on the existing and possible countermeasures to address the imminent exploits of the design flaws. The results are meant to be used as guidelines for designing and implementing secure cross-chain bridge architectures, preventing design flaws, and mitigating the negative impacts of exploits.

==> sections/background.old.tex <==
\section{Bridges (Background)} \label{sec:background}

\subsection{title}

%IT depends

Introduce background concepts:
SIDECHAIN

The first bridge
%Polygon?
zkrollup
\begin{itemize}
    \item SRA and the relevant scope
    \item Blockchain interoperability usecases and those that are useful
    \item Blockchain interoperability archirectures and those that are relevant.
\end{itemize}

\subsection{The security reference archirecture and scope}

% TODO Update figure and justify scope
% Edge cases:
% In: Bankrun, Bridge application DNS hijack
% Out: Rugpull, BGP hijack

% Categorizing bridges by different aspects Push-based Asset Transfers etc, we first tried based on compatability between chains. Not helpful. Implementing Secure Bridges: Learnings from the Secure Asset Transfer Protocol

\begin{figure}
  \centering
  \includegraphics[width=0.7\textwidth]{figures/SRAScope.png}
  \caption{The blockchain security reference architecture~\cite{9239372} with highlights on the scope of our study.}
  \label{fig:SRA}
\end{figure}

\subsection{Blockchain interoperability usecases}

% Todo: Write more about the different uses cases and different tokens to justify why we focus only on fungible tokens

There can be several use cases for interoperability. For the purpose of our study we focus on decentralised approaches to transfer fungible tokens, including:

\begin{itemize}
    \item Exchange one token on the source chain for a different token on the destination chain.
    \item Bridging of an token on the source chain for a wrapped token on the destination chain.
\end{itemize}

The following use cases are out of scope:

\begin{itemize}
    \item Transfer non-fungible tokens
    \item Transfer data
    \item Transfer state
    \item Cross-chain function calls
\end{itemize}

However, we believe that the findings for fungible tokens can be applied to a broader set of use cases, including those out of scope. We will address this as we discuss our findings.

\subsection{Blockchain interoperability solutions}

Different definitions for blockchain interoperability ~\cite{10.1145/3471140, Bridges-Between-Islands-Cross-Chain-Technology, ethereumBridgeDefinitions} presents a soup of ways to understand interoperability. The practical implementations might look different from the definitions or appear as a mixed implementation, e.g.,~\cite{multichainInteroperability}.

% TODO: We decide which categories that are more relevant after making our own assesment and comparing it to the theories.

%Based on~\cite{10.1145/3471140} we include:

%\begin{itemize}
%    \item Sidechains \& Relays
%    \item Notary Scheme (decentralised)
%    \item HTLC
%    \item Blockchain of Blockchains
%    \item Trusted Relays
%    \item Blockchain agnostic protocols
%\end{itemize}

%Based on~\cite{10.1145/3471140} we exclude:

%\begin{itemize}
%    \item Notary Scheme (centralised)
%    \item Blockchain Migrators
%\end{itemize}

%Based on~\cite{Bridges-Between-Islands-Cross-Chain-Technology} we include:

%\begin{itemize}
%    \item Manual asset exchange
%    \item Notary Scheme (decentralised)
%    \item Sidechain (Relay)
%    \item Hybrid Solution
%\end{itemize}

%Based on~\cite{Bridges-Between-Islands-Cross-Chain-Technology} we exclude:

%\begin{itemize}
%    \item Notary Scheme (centralised)
%\end{itemize}

%Based on~\cite{ethereumBridgeDefinitions} we include all the four definitions:

%\begin{itemize}
%    \item Native bridges
%    \item Validator or oracle based bridges
%    \item Generalised message passing bridges
%    \item Liquidity networks
%\end{itemize}

%Based on the practial implementaion of Multichain~\cite{multichainInteroperability} we include:

%\begin{itemize}
%    \item Bridge
%    \item Router
%\end{itemize}

%Based on the practial implementaion of Multichain~\cite{multichainInteroperability} we exclude:

%\begin{itemize}
%    \item Crosschain Contract Calls
%    \item Crosschain NFT Bridges and Router
%\end{itemize}

\subsection{DeFi concepts}
% Could be somewhere else
Miner extractable value (MEV)

\subsection{Crosschain Risk Framework - Architecture}

%https://crosschainriskframework.github.io/

The authors of the Crosschain Risk Framework \cite{ccrf} have established viable definitions to further investigate cross-chain architectures and associated risks. They distinguish between three kinds of cross-chain interactions:

\begin{itemize}
    \item Asset exchange - an asset on one chain is swapped for an asset on another chain
    \item Asset transfer - an asset is "moved" from one chain to another by locking, minting and burning.
    \item General-purpose messaging enables complex tasks, including asset exchange and transfers and function calls, data transfer, and state transfer.
\end{itemize}

It is worth noting that asset exchange is usually performed by liquidity pools that handle tokens based on the same asset. That contrasts traditional exchanges where asset A is swapped for asset B. In liquidity pools, it is most typical to see that the tokens swapped represent the same asset. Suppose any swapping of assets in the process typically happens on a single chain in an intra-chain decentralised exchange. In other words, the exchange itself is not performed between two chains. Instead, the exchange happens before or after an asset moves from one chain to another.

The Crosschain Risk Framework presents a stack-based conceptual model of crosschain protocol architectures. The bottom layer is the messaging protocol, which decides the communication flow and trust assumptions. On top of that, there are liquidity networks, token bridges and coordination protocols that enable different kinds of cross-chain interactions.

\subsubsection{State validating protocols}

State validating protocols are layer 1 - layer 2 solutions that share a single source of truth in layer 1 and do not compromise on the trust assumptions of the layer 1 chain. These protocols allow the different networks to verify each other's state changes. This is the only protocol that rely on layer 1 - layer 2 infrastructure, whereas other protocols are applicable in any combination of layers.

\subsubsection{Consensus verifying protocols}

In these protocols, the different networks can verify the finality of the corresponding network. This is done either by on-chain or off-chain validation. In on-chain validation, the different networks perform light-client validation, which typically requires a Merkle proof to be submitted to a smart contract. An off-chain prover generates a SNARK proof of state finalisation and sends it to a smart contract.

\subsubsection{Third-party attestation protocols}

The third-party attestation protocols rely on one or an m-of-n group of trusted relayers. The relayers verify the validity of crosschain interactions.

\subsubsection{Optimistic protocols}

These protocols are optimistic in the way that they will assume all transactions to be valid until proven otherwise. The protocol relies on attestors to relay messages while watchers can identify fraud and submit fraud proofs to revert bogus transactions. This enables a 1-of-n trust assumption where only one honest watcher is required to prevent fraud.


==> sections/method.old.tex <==
\section{Method}
\label{sec:method}

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/method.png}
    \caption{Method}
    \label{fig:method}
\end{figure*}

The overall approach to our study is to perform a multivocal literature review (MLR)~\cite{GAROUSI2019101}. We are motivated to include gray literature because the most realistic in-depth details on security incidents in DeFi are found in security incidents reports. Additionally, the white-literature on design flaws for DeFi is severely limited.

We introduce additional three criteria to ensure that the quality of findings in gray literature can be assessed and sources are verifiable: 1) reports that can be confirmed by reviewing smart contract code and view transactions on the blockchain can be included; 2) we can include issues that are reported by several sources by source \textit{triangulation}~\cite{creswell2000determining}; 3) specifications that go through rigorous quality control such as Ethereum Improvement Proposals (EIPs)~\cite{EIP} at the \textit{final} stage bear similar quality as white literature, and can be included. All other gray literature sources that do not fit those criteria are not included. 

To ensure that we have covered all the aspects of design flaws in fungible tokens in DeFi we perform \textit{constant comparison} and \textit{snowball sampling}~\cite{corbin2014basics} of the sources and results we find and evaluate them against design flaws from traditional software development. To aid our analysis we make use of \textit{indexing}~\cite{deterding2021flexible} of the literature included in our analysis. We determine \textit{theoretical saturation}~\cite{corbin2014basics} when our analysis cease to generate additional design flaw definitions or expand our theory. We find these concepts from Grounded Theory (GT)~\cite{stol2016grounded} to be useful, although we do not claim to perfom a GT analysis, however, we find the tools useful for our approach.

% TODO:
Relevant things to include: Why are the google results so small - because of the google search limitations. The security incident reports seem much more interesting than the google search. Google is "just in case".

We have another researcher to make quality assesment. We use security audits to verify our definitions and design flaws. We dont include samples after 31st May, be the new ones can be used for evaluation.

%White literature serach links:
%https://www.webofscience.com/wos/woscc/summary/cf59482d-1bea-47b5-849a-983fcca13d61-90630243/date-descending/1
%https://www.scopus.com/results/results.uri?sort=plf-f&src=s&sid=e3b3a548af3d3311a192e528d1eff142&sot=a&sdt=a&sl=1148&s=TITLE-ABS-KEY%28%28blockchain+OR+%28distributed+AND+ledger%29+OR+DLT+OR+cryptoasset+OR+cryptocurrency+OR+cryptocurrencies%29+AND+%28%28front+AND+run%29+OR+%28flash+AND+loan%29+OR+%28miner+AND+extracted+AND+value%29+OR+mev+OR+hack+OR+exploit+OR+security+OR+vulnerability+OR+vulnerabilities+OR+incident+OR+attack+OR+manipulate+OR+manipulation%29%29+AND+TITLE%28notary+OR+%28automated+AND+market+AND+maker%29+OR+AMM+OR+%28side+AND+chain%29+OR+HTLC+OR+%28hash+AND+time+AND+lock+AND+contract%29+OR+%28cross+AND+chain%29+OR+%28%28decentralized+OR+decentralised%29+AND+finance%29+OR+DEFI+OR+swap+OR+%28%28crypto+OR+cryptocurrency+OR+cryptocurrencies+OR+cryptoasset+OR+cryptoassets+OR+decentralized+OR+decentralised+OR+centralized+OR+centralised%29+AND+exchange%29+OR+CEX+OR+DEX+OR+bridge+OR+bridging+OR+%28wrapped+AND+token%29+OR+WBTC+OR+WETH+OR+%28liquidity+AND+pool%29+OR+%28inter+AND+chain%29+OR+interoperability+OR+interoperable%29+AND+NOT+TITLE%28seismic+OR+health+OR+healthcare+OR+NFT+OR+supply+OR+%28smart+AND+city%29+OR+EHR+OR+EMR+OR+enterprise+OR+%28data+AND+transfer%29+OR+medical+OR+%28data+AND+sharing%29+OR+e-health+OR+ehealth+OR+pharmaceutical+OR+patient+OR+iot+OR+agriculture+OR+food+OR+%28identity+AND+management%29+OR+scam+OR+fraud%29&origin=savedSearchNewOnly&txGid=6f97a78ed98a57c542b2f2133712cabb&sessionSearchId=e3b3a548af3d3311a192e528d1eff142&limit=10

The gray literature archives were chosen because\dots
% Certic and immuniefi makes incident reports
% https://github.com/immunefi-team/Web3-Security-Library?utm_source=immunefi
% https://wooded-meter-1d8.notion.site/0e85e02c5ed34df3855ea9f3ca40f53b?v=22e5e2c506ef4caeb40b4f78e23517ee
% https://github.com/immunefi-team/Web3-Security-Library/blob/main/BugFixReviews/README.md#2021
% https://github.com/immunefi-team/Web3-Security-Library/blob/main/Vulnerabilities/README.md
% https://github.com/SunWeb3Sec/DeFiHackLabs
% https://github.com/SunWeb3Sec/DeFiVulnLabs
% Security incident reports
% https://www.certik.com/resources/blog/2aHoafYEoeRguK2gE9fD1s-hack3d-the-web3-security-report-2022
% https://www.certik.com/resources/blog/4Rt6nVfk3RZGuvLGbSCOoK-2022-year-in-review-lending-protocols
% https://www.certik.com/resources (reports)
% www.rekt.news
% https://www.halborn.com/blog/category/explained-hacks
% https://www.halborn.com/blog/category/year-in-review
% https://www.halborn.com/blog/category/month-in-review
% https://beosin.com/resources?lang=en-US (security incident and research report)
% https://go.chainalysis.com/2023-crypto-crime-report-thank-you.html?aliId=eyJpIjoiZUo3OUpiT25xUW9hbElCXC8iLCJ0IjoibzBBeDNHdFhXOEJMbzFPNUlsWEZcL1E9PSJ9


==> sections/relatedWork.tex <==
%\section{Related Work}
\subsection{Comparison with related work}
%\label{sec:relatedWork}

Li et al.~\cite{9881607} made a security analysis of vulnerabilities, attacks, and advances in DeFi. Their results encompass:
\begin{enumerate}
  \item Vulnerability categories:
  \begin{itemize}
    \item Data security
    \item Consensus mechanism
    \item Smart contract
    \item Application layer
  \end{itemize}
  \item Attacks:
  \begin{itemize}
    \item Utilization of Flash Loan
    \item Private Key Leakage
    \item Reentry attack
    \item Arithmetic bug
    \item Other Bugs
  \end{itemize}
  \item Optimizations:
  \begin{itemize}
    \item Data Security Optimization
    \item Smart Contract Security Optimization
    \item Consensus Layer Optimization
    \item P2P Network Optimization 
    \item Application Layer Optimization 
  \end{itemize}
\end{enumerate}
Their analysis has a different approach compared to our work and does not focus on design flaws and solutions. However, we argue that their results encompass five different design flaws and three partly corresponding solutions. The results from Li et al.~is a good starting point in our endeavor to create comprehensive developer security guidelines covering design flaws in DeFi.

Homoliak et al.~\cite{9239372} presents a comprehensive security reference architecture. Their reference architecture is helpful to get an overview of all possible security perspectives in blockchain. On the other hand, when it comes to cross-chain design flaws, we argue that Homoliak's results become too superficial, and often propose solutions from angles inaccessible to DeFi developers. For instance, the threat of smart contract specific bugs should be addressed using safe languages, best practices, and design patterns. In our analysis, we go into depth on best practices and design patterns to present developers with a more precise guide for secure cross-chain development.
In the case of angles inaccessible to DeFi developers, Homoliak et al.~suggest solutions to handle front-running. However, their proposed solutions are only viable by changing blockchain protocols. DeFi developers do usually not have the privilege to change blockchain protocols to their liking and need other techniques to handle these issues from the perspective of their cross-chain services.

Lee et al.~\cite{10174993} present a systematization of knowledge solely focused on bridge hacks. We argue that all the six hacks and solutions they present correspond to pairs of six design flaws and solutions. For future work, the authors suggest more efforts to study preventative measures for the hacks they present. Our analysis seeks to improve guidelines for preventative measures as well as a more comprehensive guide. We observe that many cross-chain services offer a mix of bridges and exchanges, and we want to cover all the viable aspects for cross-chain engineers.

Haugum et al.~\cite{10.1145/3530019.3531345} present 16 key vulnerabilities and partly corresponding mitigation techniques in blockchain interoperability. We argue that their results are most relevant for developers who build the underlying infrastructure, i.e., blockchains, not those who utilize the infrastructure to implement DeFi solutions. Furthermore, their work is not correlated with real-world attacks and has superficial descriptions of the mitigation approaches for the vulnerabilities.  

%We want to show a different level of abstraction to provide a reference for developers to avoid creating vulnerable services in DeFi. 

% Todo: Write about these and justify novelty.
%- More incidents -> More flaws/optimizations
%- Different abstraction level, how is it different?

%Security Analysis of DeFi: Vulnerabilities, Attacks and Advances 
%https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9881607
%- This paper is very good

%The Security Reference Architecture for Blockchains: Toward a Standardized Model for Studying Vulnerabilities, Threats, and Defenses
%https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9239372
%- Its comprehensive and impressive. OTOH, too superficial for my purpose. The defence method for smart contract i for instance to follow best practices and design patterns. However, where are they? - I will make them.

%SoK: Not Quite Water Under the Bridge: Review of Cross-Chain Bridge Hacks
%https://arxiv.org/abs/2210.16209
%Its about vulnerability categorization and solutions.
%The approach seems ad-hoc and the solutions might be incomplete
%The reults dont work well as a reference guide.

%Other (attack detection):
%https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9402298
%https://dl.acm.org/doi/abs/10.1145/3551349.3559520
%xScope, blockeye
% Detection of some specific attacks
% Not design and prevention.

%Security and Privacy Challenges in Blockchain Interoperability - A Multivocal Literature Review
%https://dl.acm.org/doi/pdf/10.1145/3530019.3531345

%A Survey on Ethereum Systems Security: Vulnerabilities, Attacks, and Defenses
%https://dl.acm.org/doi/pdf/10.1145/3391195
% It is apparently not related work they say because its not crosschain. I believe there are many similarities.


==> sections/results.old.tex <==
\section{Results}
\label{sec:results}

We sorted all the inspected bridges according to the crosschain communication protocol stack to understand the causal connections between architectures and exploits. The categorization can be seen in~\cref{fig:solutionsCategories} [ERROR in creference], where bridges are arranged by communication protocol X bridge type.

Our approach has been to search for bridges that have been exploited. Therefore, the representation is most complete for those marked by red frames. On the other hand, some bridges have likely not been included in this study because there has not been an effective exploit of those bridges. 

Another detail indicated in the figure is that two types of liquidity networks are relevant to the study. The most common implementations are liquidity networks where the same assets are equal on all chains, such as Poly Network, and these assets are only transferred in a 1:1 fashion between chains. This requires no price calculation of the asset transfer. In contrast, cross-chain exchanges, such as ThorChain, using liquidity networks have additional complexity.

%Does these *same* asset liquidity network desire a label? Like "1:1 liquidity network"

\begin{figure*}
  \centering
  \includegraphics[width=1\textwidth]{figures/solutionsCategories.png}
  \label{fig:solutionsCategoriesOld}
  \caption{Categorisation of different bridges. The grid comprises the communication protocols as columns and bridge types as rows. The grid shows all the bridges considered during this study but is not necessarily an exhaustive collection of bridges. Three kinds of borders indicate whether the bridges have been exploited: 1) Bridges with a solid red frame have been exploited. 2) Bridges with a dashed cyan frame had known vulnerabilities that were fixed before being exploited. 3) Bridges with a pink dotted frame have been exploited. However, the vulnerabilities were out of scope because they were related to other components, such as arbitrage between single-chain swaps.}
\end{figure*}


% The Rainbow bridge suggests that bridge pairs shouldn't be identical depending on the direction they travel and what control the bridge operators has over the chain.

% 1:1 liquidity networks and others.

% burn and mint

% Limitation: Have not made an effort to find reported bugs that were not exploited. Some bridges are not included because they were not discovered or sought after.

% make a distinction between authentication bypass and forging signature.

% Should solutions/improvement/enhancement be described per vulnerability, per component, or separately? I think separately.

